Adaptive Self-training for Few-shot Neural Sequence Labeling

Sequence labeling is an important technique employed for many Natural Language Processing (NLP) tasks, such as Named Entity Recognition (NER), slot tagging for dialog systems and semantic parsing. Large-scale pre-trained language models obtain very good performance on these tasks when fine-tuned on large amounts of task-specific labeled data. However, such large-scale labeled datasets are difficult to obtain for several tasks and domains due to the high cost of human annotation as well as privacy and data access constraints for sensitive user applications. This is exacerbated for sequence labeling tasks requiring such annotations at token-level. In this work, we develop techniques to address the label scarcity challenge for neural sequence labeling models. Specifically, we develop self-training and meta-learning techniques for training neural sequence taggers with few labels. While self-training serves as an effective mechanism to learn from large amounts of unlabeled data -- meta-learning helps in adaptive sample re-weighting to mitigate error propagation from noisy pseudo-labels. Extensive experiments on six benchmark datasets including two for massive multilingual NER and four slot tagging datasets for task-oriented dialog systems demonstrate the effectiveness of our method. With only 10 labeled examples for each class for each task, our method obtains 10% improvement over state-of-the-art systems demonstrating its effectiveness for the low-resource setting.

==> subfiles/extra_results.tex <==

\begin{table}[ht]
\centering
\caption{Variation in model performance on varying $K$ labels / slot on SNIPS dataset with $39$ slots.} 
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots }\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT(Full) & 0.9580 & 0.9580 & 0.9580 & 0.9580\\
\midrule
BERT(base) & 0.7063 & 0.7901 &  0.8681& 0.9390\\
CVT & 0.6982 & 0.7823 & 0.8804 & 0.9461\\
SeqVAT & 0.6934& 0.7867 & 0.8505 & 0.9146  \\
Mean Teacher &0.7085 &0.7948 & 0.8731 & 0.9426\\
VAT & 0.7134 & 0.7908& 0.8819&0.9453\\
Classic ST & 0.7259 & 0.8326 & 0.8832 & 0.9392 \\
BOND & 0.7285 & 0.8354 & 0.8893 & 0.9422\\
\midrule
MetaST & 0.8156 (\textcolor{red}{$\uparrow$15\%}) &0.8822 (\textcolor{red}{$\uparrow$12\%}) &0.9199 (\textcolor{red}{$\uparrow$6\%}) &0.9539 (\textcolor{red}{$\uparrow$2\%})\\
\bottomrule
\end{tabular}
\label{tab:snips}
}

\end{table}


\begin{table}[ht]
\centering
\caption{The performance changes wrt. K shots on CONLL2003}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (4 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 63.87 & 70.71/71.59 & 73.57 &84.36\\
BERT(Full) & 92.40  & 92.40 & 92.40 & 92.40\\
\midrule
CVT & 51.15 &54.03 /54.58 &66.11&81.99\\
SeqVAT & 58.02 & 68.59/69.14/66.37&74.15&82.20\\
Mean Teacher &59.04 & 68.67 /68.68  &72.62&84.17\\
VAT & 57.03 & 65.89/64.17&72.69&84.43\\
Classic ST & 64.04 & 69.78/72.21 &74.65&84.93 \\
BOND &62.52  & 67.79/71.32 &74.19&83.87\\
\midrule
MetaST &71.49&75.48/75.00/75.62 & 78.54 \\

\bottomrule
\end{tabular}
}

\end{table}


	
\begin{table*}[htb!]
\centering
  \small
	\caption{F1 score comparison of different models for sequence labeling tasks on different datasets. All models (except CVT and SeqVAT) use the same BERT-Base encoder. All models (except `Fully supervised') are trained with $10$ labeled samples per slot. The F1 number for each task is followed by the
 standard deviation in parentheses and percentage improvement ($\uparrow$) over the base model.}
	\label{tab:main_result}
			\resizebox{\columnwidth}{!}{%
			\begin{tabular}{lcccccc}
				\midrule
				Method & SNIPS & Enterprise Email &  Movie & Restaurant& CONLL03 & Wikiann \\
			\midrule
				\textbf{\# of Slots}
				& 39 & 20 & 12 & 8 & 4 & 3 
				\\
				\midrule				\multicolumn{6}{l}{\textbf{Full-supervision}}\\
				BERT &95.80 & 94.44 & 87.87 & 78.95 & 92.40 & 84.04\\
				\midrule
	             \multicolumn{6}{l}{\textbf{Few-shot supervision (10 labels per slot)}}\\
					BERT & 79.01 &  87.85 & 69.50 (1.35) & 54.06 & 71.15(0.4) & 45.61\\
				\midrule
			\multicolumn{6}{l}{\textbf{Few-shot semi-supervision (10 labels per slot + unlabeled data)} }\\
				 CVT &78.23&  78.24& 62.73 &42.57 &  54.31 (0.27)   &   27.89\\
                 SeqVAT& 78.67 &72.65 &  67.1 (0.7)  & 51.55 & 67.21(1.38) & 35.16\\
                 MT & 79.48 &89.53  & 67.62 (2) & 51.75 & 68.67 (0.13) & 41.43 \\
                 VAT  & 79.08   &89.71   & 70.17 (1.07) & 53.34 & 65.03 (0.86)  & 38.81\\
                 Classic ST  & 83.26   &90.70 & 71.88(1)& 56.80  & 70.99 (1.20) & 46.15 \\
                 BOND & 83.54 &89.75 & 70.91 (1.32) & 55.78  & 69.56 (1.76) & 48.73 \\
                 \midrule
				 \multicolumn{6}{l}{\textbf{Our framework}} \\
				 MetaST& 88.23 (0.04) {($\uparrow$12\%)} & 92.18 & 77.67   &63.83(1.62)  &  75.48  & 56.61(0.4)\\
				\hline
			\end{tabular}
		    }
\label{tab:10_shot}
\end{table*}

% i)                    Appendix with all the experimental configurations like batch size, dropout, and other hyper-parameters

% ii)                   We should anonymize and submit the code for them to run

% iii)                 All experimental tables the we cannot fit in main text should go to the Appendix. Do not leave out any experimental result that you have already done.

% iv)                 For the multi-lingual datasets, we should report the per-language f-score.

\subsection{Hyper-parameter}

\subsection{K-shots}

\subsection{Multilingual}


% \begin{table*}[htb!]
% \centering
%   \small
% 	\caption{F1 score comparison of different models for sequence labeling tasks on different datasets. All models (except CVT and SeqVAT) use the same BERT-Base encoder. All models (except `Fully supervised') are trained with $10$ labeled samples per slot. The F1 number for each task is followed by the
%  standard deviation in parentheses and percentage improvement ($\uparrow$) over the base model.}
% 	\label{tab:main_result}
% 			\resizebox{\columnwidth}{!}{%
% 			\begin{tabular}{lcccccc}
% 				\midrule
% 				Method & SNIPS & Enterprise Email &  Movie & Restaurant& CONLL03 & Wikiann \\
% 			\midrule
% 				\textbf{\# of Slots}
% 				& 39 & 20 & 12 & 8 & 4 & 3 
% 				\\
% 				\midrule
% 				BERT(Base) & 79.01 &  87.85 & 69.50 (1.35) & 54.06 & 71.15(0.4) & 45.61\\
% 				\midrule
% 				\multicolumn{6}{l}{\textbf{Fully-supervised}}\\
% 				BERT &95.80 & 94.44 & 87.87 & 78.95 & 92.40 & 84.04\\
% 				\midrule
% 				\multicolumn{6}{l}{\textbf{Semi-supervised} }\\
% 				 CVT &78.23&  78.24& 62.73 &42.57 &  54.31 (0.27)   &   27.89\\
%                  SeqVAT& 78.67 &72.65 &  67.1 (0.7)  & 51.55 & 67.21(1.38) & 35.16\\
%                  MT & 79.48 &89.53  & 67.62 (2) & 51.75 & 68.67 (0.13) & 41.43 \\
%                  VAT  & 79.08   &89.71   & 70.17 (1.07) & 53.34 & 65.03 (0.86)  & 38.81\\
%                  Classic ST  & 83.26   &90.70 & 71.88(1)& 56.80  & 70.995 (1.2) & 46.15 \\
%                  BOND & 83.54 &89.75 & 70.91 (1.32) & 55.78  & 69.56 (1.76) & 48.73 \\
%                  \midrule
% 				 \multicolumn{6}{l}{\textbf{Our framework}} \\
% 				 MetaST& 88.23 (0.04) & 92.18 & 77.67   &63.83(1.62)  &  75.48  & 56.61(0.4)\\
% 				\hline
% 			\end{tabular}
% 		    }
% \end{table*}


\begin{table*}[htb!]
\centering
	\label{tab:main_result}
			\resizebox{\columnwidth}{!}{%
			\begin{tabular}{lcccccc}
				\midrule
				Method & SNIPS &  Email &  Movie & Restaurant& CONLL03 (EN) & Wikiann (EN) \\
			\midrule
				\textbf{\# of Slots}
				& 39 & 20 & 12 & 8 & 4 & 3 
				\\
				\midrule				\multicolumn{6}{l}{\textbf{Full-supervision}}\\
				BERT &95.80 & 94.44 & 87.87 & 78.95 & 92.40 & 84.04\\
				\midrule
	             \multicolumn{6}{l}{\textbf{Few-shot supervision (10 labels per slot)}}\\
					BERT & 79.01 &  87.85 & 69.50 (1.35) & 54.06 & 71.15(0.4) & 45.61\\
				\midrule
			\multicolumn{6}{l}{\textbf{Few-shot semi-supervision (10 labels per slot + unlabeled data)} }\\
				 CVT &78.23&  78.24& 62.73 &42.57 &  54.31 (0.27)   &   27.89\\
                 SeqVAT& 78.67 &72.65 &  67.1 (0.7)  & 51.55 & 67.21(1.38) & 35.16\\
                 MT & 79.48 &89.53  & 67.62 (2) & 51.75 & 68.67 (0.13) & 41.43 \\
                 VAT  & 79.08   &89.71   & 70.17 (1.07) & 53.34 & 65.03 (0.86)  & 38.81\\
                 Classic ST  & 83.26   &90.70 & 71.88(1)& 56.80  & 70.99 (1.20) & 46.15 \\
                 BOND & 83.54 &89.75 & 70.91 (1.32) & 55.78  & 69.56 (1.76) & 48.73 \\
                 \midrule
				 \multicolumn{6}{l}{\textbf{Our framework}} \\
				 MetaST& 88.23 (0.04) {($\uparrow$12\%)} & 92.18 {($\uparrow$4.93\%)}& 77.67  {($\uparrow$11.76\%)} &63.83(1.62) {($\uparrow$18.07\%)} &  76.65 (0.73)  {($\uparrow$7.73\%)}& 56.61(0.4) {($\uparrow$24.12\%)}\\
				\hline
			\end{tabular}
		    }
		   	\caption{F1 score comparison of different models for sequence labeling tasks on different datasets. All models (except CVT and SeqVAT) use the same BERT-Base encoder. The F1 score for each task is followed by the standard deviation in parentheses and percentage improvement ($\uparrow$) over the BERT model with few-shot supervision.}
\label{tab:10_shot}
\end{table*}



\begin{table}[ht]
\centering
\caption{Email Dataset.} 
\resizebox{0.3\linewidth}{!}{
\begin{tabular}{c|cc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{2}{c}{Shots}\\

\cline{2-3}
 & 
5  & 10 \\
\midrule
\midrule
BERT(base) & 0.8211 & 0.8785 \\
BERT(Full) & 0.9444 & 0.9444 \\
\midrule
CVT & 67.44& 78.24 \\
SeqVAT & 64.67 & 72.65\\

Mean Teacher & 84.10&89.53  \\
VAT &  83.24& 89.71\\
Classic ST & 86.88 & 90.70  \\

BOND & 84.92 & 89.75\\
\midrule
MetaST & 89.21 &92.18\\

\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[ht]
\centering
\caption{SNIPS Dataset.} 
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (39 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT(base) & 0.7063 & 0.7901 &  0.8681& 0.9390\\
BERT(Full) & 0.9580 & 0.9580 & 0.9580 & 0.9580\\
\midrule
CVT & 0.6982 & 0.7823/79.16 & 0.8804 & 0.9461\\
SeqVAT & 0.6934& 0.7867 & 0.8505 & 0.9146  \\
Mean Teacher &0.7085 &0.7948 & 0.8731 & 0.9426\\
VAT & 0.7134 & 0.7908& 0.8819&0.9453\\
Classic ST & 0.7259 & 0.8326 & 0.8832 & 0.9392 \\
BOND & 0.7285 & 0.8354 & 0.8893 & 0.9422\\
\midrule
MetaST & 0.8156 (\textcolor{red}{$\uparrow$15\%}) &0.8822/0.8830 (\textcolor{red}{$\uparrow$12\%}) &0.9199 (\textcolor{red}{$\uparrow$6\%}) &0.9539 (\textcolor{red}{$\uparrow$2\%})\\
\bottomrule
\end{tabular}
}

\end{table}

% \begin{table}[htb]
% \centering
% \caption{MIT Movie Dataset.} 
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|cccc}
% \toprule

% \multirow{2}{*}{Method} &
% \multicolumn{4}{c}{Shots (12 Slot  Types)}\\

% \cline{2-5}
%  & 
% 5  & 10 & 20 & 100\\
% \midrule
% \midrule
% BERT(base) & 0.5175 & 0.5348 & 0.6597 &  0.7108\\
% BERT (Full) & 0.8787 & 0.8787 & 0.8787 & 0.8787\\
% \midrule
% CVT &0.4117 & 0.4401& 0.5163 & 0.6554\\
% SeqVAT & 0.4783 & 0.5370 & 0.6271 & 0.6911 \\
% Mean Teacher & 0.4727 & 0.5324 & 0.6356 & 0.7054\\
% VAT & 0.4729 & 0.5149 & 0.6447 & 0.6944\\

% Classic ST & 0.5343 & 0.5684 &0.6774 & 0.7109 \\
% BOND & 0.5038 &  0.5561 & 0.6627 & 0.7109 \\
% \midrule
% MetaST & 0.5505&0.5923 &0.6777 & 0.7386\\
% \bottomrule
% \end{tabular}
% }

% \end{table}






\begin{table}[ht]
\centering
\caption{MIT Movie Dataset.} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (12 Slot  Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT(base) & 0.6280 & 69.50 (1.35) & 0.7581 & 0.8249\\
BERT (Full) & 0.8787 & 0.8787 & 0.8787 & 0.8787\\
\midrule
CVT & 57.48 &  62.73&70.20&81.82 \\
SeqVAT & 60.94 & 67.1(0.7) & 74.15 & 82.73\\
Mean Teacher & 58.92 & 67.62 (2) & 0.7524 & 0.8220\\
VAT & 0.6075 & 70.17(1.07) & 0.75413 & 0.8239\\

Classic ST & 0.6339 & 71.88 (1) & 0.7658 & 0.8306\\
BOND & 0.6250 & 70.91 (1.32) & 0.7552 & 0.8265\\
\midrule
MetaST & 72.57 & 77.67/ 77.44/77.59 &80.33 & 84.35 \\
\bottomrule
\end{tabular}
}

\end{table}




\begin{table}[ht]
\centering
\caption{MIT Restaurant Dataset.} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (8 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT(base) & 0.4139 & 0.5406/56.49 & 0.6012 & 0.7224\\
BERT(Full) & 0.7895 & 0.7895 & 0.7895 & 0.7895\\
\midrule
CVT &0.3374 &0.4257/41.89 & 0.5133 &0.7084\\
SeqVAT & 0.4194 & 0.5155 & 0.5615 & 0.7139\\
Mean Teacher & 0.4037 & 51.75/54.88 & 0.5734 & 0.7240\\
VAT & 0.4129 & 53.34/55.42 & 0.5968 & 0.7265 \\
Classic ST & 0.4435 & 0.5680/57.49& 0.6028 & 0.7313 \\
BOND & 0.4301 &  0.5578/56.87 &  0.5996 & 0.7360 \\
\midrule
MetaST &0.5302 & 63.21/64.58/65.33& 67.86 &  0.7525\\

\bottomrule
\end{tabular}
}

\end{table}

% \begin{table}[htb]
% \centering
% \caption{CONLL2003 Dataset (English).} 
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|cccc}
% \toprule

% \multirow{2}{*}{Method} &
% \multicolumn{4}{c}{Shots (4 Slot Types)}\\

% \cline{2-5}
%  & 
% 5  & 10 & 20 & 100\\
% \midrule
% \midrule
% BERT (base) & 0.5457 & 0.5849 & 0.6606 & 0.7768\\
% BERT(Full) & 0.9240  & 0.9240 & 0.9240 & 0.9240\\
% \midrule
% CVT &0.4217 &0.5266 &  0.5590& 0.7074\\
% SeqVAT & 0.3641 & 0.4195 & 0.5341&0.7416\\
% Mean Teacher & 0.5342 & 0.5596 & 0.6509 & 0.7825\\
% VAT & 0.5155 & 0.5618 & 0.6399 & 0.7761\\
% Classic ST & 0.5972 & 0.6299 &  0.7099 & 0.8242\\
% BOND & 0.6040 &  0.6185 & 0.6937 & 0.8158  \\
% \midrule
% MetaST & 0.6094 &\textcolor{red}{0.6584}\\

% \bottomrule
% \end{tabular}
% }

% \end{table}



\begin{table}[ht]
\centering
\caption{The performance changes wrt. K shots on CONLL2003}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (4 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 63.87 & 68.70.71/71.59 & 73.57 &84.36\\
BERT(Full) & 92.40  & 92.40 & 92.40 & 92.40\\
\midrule
CVT & 51.15 &54.03 /54.58 &66.11&81.99\\
SeqVAT & 58.02 & 68.59/69.14/66.37&74.15&82.20\\
Mean Teacher &59.04 & 68.67 /68.68  &72.62&84.17\\
VAT & 57.03 & 65.89/64.17&72.69&84.43\\
Classic ST & 64.04 & 69.78/72.21 &74.65&84.93 \\
BOND &62.52  & 67.79/71.32 &74.19&83.87\\
\midrule
MetaST &71.49&75.48/77.11/75.62 & 78.54 & 85.77 \\

\bottomrule
\end{tabular}
}

\end{table}


\begin{table}[ht]
\centering
\caption{Wikiann Dataset (English).} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (3 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 37.01 & 45.61 & 54.53 & 67.87\\
BERT(Full) & 84.04   & 84.04  & 84.04 & 84.04 \\
\midrule
CVT &16.05 & 27.89/29.75 & 46.42&66.36\\
SeqVAT & 21.11 & 35.16&42.26&62.37\\
Mean Teacher & 30.92 & 41.43 & 50.61 & 67.16\\
VAT & 24.72 & 38.81 & 50.15 & 66.31\\
Classic ST & 32.72 & 46.15 & 54.41 & 68.64\\
BOND & 34.22 & 48.73 & 52.45 & 68.89 \\
\midrule
MetaST &55.04& 57.01/52.18/59.31 & 60.38 & 73.20\\

\bottomrule
\end{tabular}
}

\end{table}




\begin{table}[ht]
\centering
\caption{Multilingual CONLL2003 Dataset.} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (4 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 0.6480 & 0.7077/72.33 & 0.7389 & 0.8061 \\
BERT(Full) & 0.8767 & 0.8767& 0.8767 & 0.8767 \\
\midrule

Mean Teacher & 0.6455 &0.6834&0.7387&0.7921\\
VAT &0.6497 & 0.6763 & 0.7426 & 0.8070  \\
Classic ST &0.6795 &  0.7269&0.7379&0.8182\\
BOND & 0.6942 & 0.7279 & 0.7602 & 0.8062  \\
\midrule
MetaST &0.7334 &  \textcolor{red}{75.01} & 77.01 & 82.11\\

\bottomrule
\end{tabular}
}

\end{table}

\begin{table}[ht]
\centering
\caption{Multilingual Wikiann Dataset.} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (3 Slot Types $\times$ 41 languages)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 0.7768 & 0.7967/77.02/77.35 & 0.8233 & 0.8570 \\
BERT(Full) &  0.8717 &  0.8717 &  0.8717 & 0.8717 \\
\midrule

Mean Teacher & 0.7709 & 0.8023 & 0.8219 & 0.8534\\
VAT & 0.7471 & 0.7882 & 0.8260 & 0.8582\\
Classic ST & 0.7673  & 0.8024 & 0.8239 & 0.8608\\
BOND & 0.7881 & 0.7957 & 0.8219&0.8614 \\
\midrule
MetaST &79.10& 81.47/81.75/81.11 & 83.14 & 85.57\\

\bottomrule
\end{tabular}
}

\end{table}



% The optimal $\epsilon^{*}$ is given by:

% \begin{equation}
%     \epsilon_{m, n, k} = \argmin_{\epsilon_{m, n}}  \big ( \frac{1}{{|\mathcal{B}^l_k|}} \frac{1}{N} \sum_{m=1}^{|\mathcal{B}^l_k|} \sum_{n=1}^{N} [ l(y_{m, n}, f(x_{m, n}; \hat{\theta}^{(t)}_{stu} (\epsilon))] \big )
% \end{equation}
\begin{table*}[htb!]
\vspace{-0.1in}
\small

\centering
	\label{tab:main_result}
	\resizebox{\columnwidth}{!}{%
			\begin{tabular}{lcccccc}
				\midrule
				Method & SNIPS &  Email &  Movie & Restaurant& CoNLL03 (EN) & Wikiann (EN) \\
			\midrule
				\textbf{\# Slots}
				& 39 & 20 & 12 & 8 & 4 & 3 
				\\
				\midrule				\multicolumn{6}{l}{\textbf{Full-supervision}}\\
				BERT &95.80 & 94.44 & 87.87 & 78.95 & 92.40 & 84.04\\
				\midrule
	             \multicolumn{6}{l}{\textbf{Few-shot supervision (10 labels per slot)}}\\
					BERT & 79.01 &  87.85 & 69.50 (1.35) & 54.06 & 71.15(0.4) & 45.61\\
				\midrule
			\multicolumn{6}{l}{\textbf{Few-shot supervision (10 labels per slot) + unlabeled data} }\\
				 CVT &78.23&  78.24& 62.73 &42.57 &  54.31 (0.27)   &   27.89\\
                 SeqVAT& 78.67 &72.65 &  67.1 (0.7)  & 51.55 & 67.21(1.38) & 35.16\\
                 MT & 79.48 &89.53  & 67.62 (2) & 51.75 & 68.67 (0.13) & 41.43 \\
                 VAT  & 79.08   &89.71   & 70.17 (1.07) & 53.34 & 65.03 (0.86)  & 38.81\\
                 Classic ST  & 83.26   &90.70 & 71.88(1)& 56.80  & 70.99 (1.20) & 46.15 \\
                 BOND & 83.54 &89.75 & 70.91 (1.32) & 55.78  & 69.56 (1.76) & 48.73 \\
                 \midrule
				% \multicolumn{6}{l}{\textbf{Our framework}} \\
				 MetaST& 88.23 (0.04) {($\uparrow$12\%)} & 92.18 {($\uparrow$4.93\%)}& 77.67  {($\uparrow$11.76\%)} &63.83(1.62) {($\uparrow$18.07\%)} &  76.65 (0.73)  {($\uparrow$7.73\%)}& 56.61(0.4) {($\uparrow$24.12\%)}\\
				\hline
			\end{tabular}
		    }
		   	\caption{F1 score comparison of different models for sequence labeling tasks on different datasets. All models (except CVT and SeqVAT) use the same BERT-Base encoder. The F1 score for each task is followed by the standard deviation in parentheses and percentage improvement ($\uparrow$) over the BERT model with few-shot supervision.}
\label{tab:10_shot_f}
\vspace{-0.2in}
\end{table*}




% i)                    Appendix with all the experimental configurations like batch size, dropout, and other hyper-parameters

% ii)                   We should anonymize and submit the code for them to run

% iii)                 All experimental tables the we cannot fit in main text should go to the Appendix. Do not leave out any experimental result that you have already done.

% iv)                 For the multi-lingual datasets, we should report the per-language f-score.


\begin{figure}[hb]
\centering
\small
\vspace{-0.2in}
\begin{minipage}{0.48\textwidth}
\centering
\captionsetup{type=table} %% tell latex to change to table
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{c|c|c}
\toprule
\multirow{2}{*}{Ratio of Unlabeled Data} &
\multicolumn{2}{c}{Datasets}\\
\cline{2-3}
 & 
SNIPS  & CoNLL03 \\
\midrule
\midrule
%0.05\% & & \\
5\% & 84.47 & 72.92\\
25\% &87.10 &  76.46\\
%50\% & 86.60&  75.43\\
75\% &87.50 & 76.56\\
\bottomrule
\end{tabular}
}
\caption{Varying proportion of unlabeled data for MetaST with 10 labels per slot.} % The $0.05\%$ and $5\%$ of unlabeled data are similar with CoNLL03 and SNIPS 10 labeled data sizes respectively.
\label{tab:ablation_unlabeled_data}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\centering
\captionsetup{width=0.7\textwidth}
	\includegraphics[width=0.65\textwidth]{figs/varying_minibatches.eps}
 	   \vspace{-0.5em}	\caption{Varying $S$ mini-batch labeled data for re-weighting.}
 	 \label{fig:ablation_minibatch}
\end{minipage}
\end{figure}


\noindent {\bf Variation in model performance with unlabeled data.} Table~\ref{tab:ablation_unlabeled_data} shows the improvement in model performance as we inject more unlabeled data with diminishing returns after a certain point.

%, we also observe diminishing returns on  While a decent amount of unlabeled data helps the model toBy varying size of unlabeled data for semi-supervised learning, we can clearly observe that model gets better performance with more unlabeled data. }

% \begin{table}[ht]
% \centering
% \caption{Varying Unlabeled Data.} 
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|c|c|c}
% \toprule

% \multirow{2}{*}{Size of Unlabeled Data} &
% \multicolumn{2}{c}{Datasets}\\

% \cline{2-4}
%  & 
% SNIPS  & Conll &  Wikiann\\
% \midrule
% \midrule
% 25\% &86.10 &  \\
% 50\% & 86.60&  \\
% 75\% &87.50 & \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:ablation_unlabeled_data}
% \end{table}



\noindent {\bf Variation in model performance with mini-batch S.} We set the value of $S$ in Eq.~\ref{Eq:meta_weight} to $\{1, 3, 5\}$ respectively to explore its impact on the re-weighting mechanism. From Figure~\ref{fig:ablation_minibatch} we observe that the model is not super sensitive to hyper-parameter $S$ but can achieve a better estimate of the weights of the pseudo-labeled data with increasing mini-batch values. 

\subsection{Analysis of Re-weighting on SNIPS and CoNll03}
\subsection{Ablation}
\label{sec:ablation}
\begin{figure}[hb]
 \vspace{-0.2in}
 \small
 \centering
\subfloat[SNIPS]{
\begin{minipage}{.48\textwidth}
\includegraphics[height=1.5in]{figs/snips_select.png}
\label{subfig:snips}
\end{minipage}}
\subfloat[CoNLL03]{
\begin{minipage}{.48\textwidth}
\includegraphics[height=1.5in]{figs/conll_select.png}
\label{subfig:conll}
\end{minipage}}
 \caption{Visualization of MetaST re-weighting examples on SNIPS and CoNLL03. (Figure to be updated.)}\label{fig:conll_select}
 \vspace{-0.1in}
\end{figure}

\subsection{Hyper-parameter}


\subsection{K-shots}



% \begin{table*}[htb!]
% \centering
%   \small
% 	\caption{F1 score comparison of different models for sequence labeling tasks on different datasets. All models (except CVT and SeqVAT) use the same BERT-Base encoder. All models (except `Fully supervised') are trained with $10$ labeled samples per slot. The F1 number for each task is followed by the
%  standard deviation in parentheses and percentage improvement ($\uparrow$) over the base model.}
% 	\label{tab:main_result}
% 			\resizebox{\columnwidth}{!}{%
% 			\begin{tabular}{lcccccc}
% 				\midrule
% 				Method & SNIPS & Enterprise Email &  Movie & Restaurant& CONLL03 & Wikiann \\
% 			\midrule
% 				\textbf{\# of Slots}
% 				& 39 & 20 & 12 & 8 & 4 & 3 
% 				\\
% 				\midrule
% 				BERT(Base) & 79.01 &  87.85 & 69.50 (1.35) & 54.06 & 71.15(0.4) & 45.61\\
% 				\midrule
% 				\multicolumn{6}{l}{\textbf{Fully-supervised}}\\
% 				BERT &95.80 & 94.44 & 87.87 & 78.95 & 92.40 & 84.04\\
% 				\midrule
% 				\multicolumn{6}{l}{\textbf{Semi-supervised} }\\
% 				 CVT &78.23&  78.24& 62.73 &42.57 &  54.31 (0.27)   &   27.89\\
%                  SeqVAT& 78.67 &72.65 &  67.1 (0.7)  & 51.55 & 67.21(1.38) & 35.16\\
%                  MT & 79.48 &89.53  & 67.62 (2) & 51.75 & 68.67 (0.13) & 41.43 \\
%                  VAT  & 79.08   &89.71   & 70.17 (1.07) & 53.34 & 65.03 (0.86)  & 38.81\\
%                  Classic ST  & 83.26   &90.70 & 71.88(1)& 56.80  & 70.995 (1.2) & 46.15 \\
%                  BOND & 83.54 &89.75 & 70.91 (1.32) & 55.78  & 69.56 (1.76) & 48.73 \\
%                  \midrule
% 				 \multicolumn{6}{l}{\textbf{Our framework}} \\
% 				 MetaST& 88.23 (0.04) & 92.18 & 77.67   &63.83(1.62)  &  75.48  & 56.61(0.4)\\
% 				\hline
% 			\end{tabular}
% 		    }
% \end{table*}




\begin{figure}[hb]
\centering
\small
\begin{minipage}{0.48\textwidth}
\centering
\captionsetup{type=table} %% tell latex to change to table
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{c|cc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{2}{c}{Shots}\\

\cline{2-3}
 & 
5  & 10 \\
\midrule
\midrule
BERT(base) & 0.8211 & 0.8785 \\
BERT(Full) & 0.9444 & 0.9444 \\
\midrule
CVT & 67.44& 78.24 \\
SeqVAT & 64.67 & 72.65\\

Mean Teacher & 84.10&89.53  \\
VAT &  83.24& 89.71\\
Classic ST & 86.88 & 90.70  \\

BOND & 84.92 & 89.75\\
\midrule
MetaST & 89.21 &92.18\\

\bottomrule
\end{tabular}
}
\caption{Email Dataset.} % The $0.05\%$ and $5\%$ of unlabeled data are similar with CoNLL03 and SNIPS 10 labeled data sizes respectively.
\label{tab:ablation_unlabeled_data}
\end{minipage}
\begin{minipage}{0.5\linewidth}
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (12 Slot  Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT(base) & 0.6280 & 69.50 (1.35) & 0.7581 & 0.8249\\
BERT (Full) & 0.8787 & 0.8787 & 0.8787 & 0.8787\\
\midrule
CVT & 57.48 &  62.73&70.20&81.82 \\
SeqVAT & 60.94 & 67.1(0.7) & 74.15 & 82.73\\
Mean Teacher & 58.92 & 67.62 (2) & 0.7524 & 0.8220\\
VAT & 0.6075 & 70.17(1.07) & 0.75413 & 0.8239\\

Classic ST & 0.6339 & 71.88 (1) & 0.7658 & 0.8306\\
BOND & 0.6250 & 70.91 (1.32) & 0.7552 & 0.8265\\
\midrule
MetaST & 72.57 & 77.67/ 77.44/77.59 &80.33 & 84.35 \\
\bottomrule
\end{tabular}
}\caption{MIT Movie Dataset.} 
\end{minipage}
\end{figure}




% \begin{table}[ht]
% \centering
% \caption{MIT Movie Dataset.} 
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|cccc}
% \toprule

% \multirow{2}{*}{Method} &
% \multicolumn{4}{c}{Shots (12 Slot  Types)}\\

% \cline{2-5}
%  & 
% 5  & 10 & 20 & 100\\
% \midrule
% \midrule
% BERT(base) & 0.6280 & 69.50 (1.35) & 0.7581 & 0.8249\\
% BERT (Full) & 0.8787 & 0.8787 & 0.8787 & 0.8787\\
% \midrule
% CVT & 57.48 &  62.73&70.20&81.82 \\
% SeqVAT & 60.94 & 67.1(0.7) & 74.15 & 82.73\\
% Mean Teacher & 58.92 & 67.62 (2) & 0.7524 & 0.8220\\
% VAT & 0.6075 & 70.17(1.07) & 0.75413 & 0.8239\\

% Classic ST & 0.6339 & 71.88 (1) & 0.7658 & 0.8306\\
% BOND & 0.6250 & 70.91 (1.32) & 0.7552 & 0.8265\\
% \midrule
% MetaST & 72.57 & 77.67/ 77.44/77.59 &80.33 & 84.35 \\
% \bottomrule
% \end{tabular}
% }

% \end{table}




\begin{figure}[hb]
\centering
\small
\begin{minipage}{0.48\linewidth}
\centering
\captionsetup{type=table} %% tell latex to change to table
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (8 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT(base) & 0.4139 & 0.5406/56.49 & 0.6012 & 0.7224\\
BERT(Full) & 0.7895 & 0.7895 & 0.7895 & 0.7895\\
\midrule
CVT &0.3374 &0.4257/41.89 & 0.5133 &0.7084\\
SeqVAT & 0.4194 & 0.5155 & 0.5615 & 0.7139\\
Mean Teacher & 0.4037 & 51.75/54.88 & 0.5734 & 0.7240\\
VAT & 0.4129 & 53.34/55.42 & 0.5968 & 0.7265 \\
Classic ST & 0.4435 & 0.5680/57.49& 0.6028 & 0.7313 \\
BOND & 0.4301 &  0.5578/56.87 &  0.5996 & 0.7360 \\
\midrule
MetaST &0.5302 & 63.21/64.58/65.33& 67.86 &  0.7525\\

\bottomrule
\end{tabular}
}
\caption{MIT Restaurant Dataset.} % 
\label{tab:ablation_unlabeled_data}
\end{minipage}
\captionsetup{type=table}
\begin{minipage}{0.48\linewidth}
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule
\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (4 Slot Types)}\\
\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 63.87 & 68.70.71/71.59 & 73.57 &84.36\\
BERT(Full) & 92.40  & 92.40 & 92.40 & 92.40\\
\midrule
CVT & 51.15 &54.03 /54.58 &66.11&81.99\\
SeqVAT & 58.02 & 68.59/69.14/66.37&74.15&82.20\\
Mean Teacher &59.04 & 68.67 /68.68  &72.62&84.17\\
VAT & 57.03 & 65.89/64.17&72.69&84.43\\
Classic ST & 64.04 & 69.78/72.21 &74.65&84.93 \\
BOND &62.52  & 67.79/71.32 &74.19&83.87\\
\midrule
MetaST &71.49&75.48/77.11/75.62 & 78.54 & 85.77 \\

\bottomrule
\end{tabular}
}\caption{The performance changes wrt. K shots on CONLL2003} 
\end{minipage}
\end{figure}


% \begin{table}[ht]
% \centering
% \caption{MIT Restaurant Dataset.} 
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|cccc}
% \toprule

% \multirow{2}{*}{Method} &
% \multicolumn{4}{c}{Shots (8 Slot Types)}\\

% \cline{2-5}
%  & 
% 5  & 10 & 20 & 100\\
% \midrule
% \midrule
% BERT(base) & 0.4139 & 0.5406/56.49 & 0.6012 & 0.7224\\
% BERT(Full) & 0.7895 & 0.7895 & 0.7895 & 0.7895\\
% \midrule
% CVT &0.3374 &0.4257/41.89 & 0.5133 &0.7084\\
% SeqVAT & 0.4194 & 0.5155 & 0.5615 & 0.7139\\
% Mean Teacher & 0.4037 & 51.75/54.88 & 0.5734 & 0.7240\\
% VAT & 0.4129 & 53.34/55.42 & 0.5968 & 0.7265 \\
% Classic ST & 0.4435 & 0.5680/57.49& 0.6028 & 0.7313 \\
% BOND & 0.4301 &  0.5578/56.87 &  0.5996 & 0.7360 \\
% \midrule
% MetaST &0.5302 & 63.21/64.58/65.33& 67.86 &  0.7525\\

% \bottomrule
% \end{tabular}
% }

% \end{table}

% \begin{table}[htb]
% \centering
% \caption{CONLL2003 Dataset (English).} 
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|cccc}
% \toprule

% \multirow{2}{*}{Method} &
% \multicolumn{4}{c}{Shots (4 Slot Types)}\\

% \cline{2-5}
%  & 
% 5  & 10 & 20 & 100\\
% \midrule
% \midrule
% BERT (base) & 0.5457 & 0.5849 & 0.6606 & 0.7768\\
% BERT(Full) & 0.9240  & 0.9240 & 0.9240 & 0.9240\\
% \midrule
% CVT &0.4217 &0.5266 &  0.5590& 0.7074\\
% SeqVAT & 0.3641 & 0.4195 & 0.5341&0.7416\\
% Mean Teacher & 0.5342 & 0.5596 & 0.6509 & 0.7825\\
% VAT & 0.5155 & 0.5618 & 0.6399 & 0.7761\\
% Classic ST & 0.5972 & 0.6299 &  0.7099 & 0.8242\\
% BOND & 0.6040 &  0.6185 & 0.6937 & 0.8158  \\
% \midrule
% MetaST & 0.6094 &\textcolor{red}{0.6584}\\

% \bottomrule
% \end{tabular}
% }

% \end{table}



% \begin{table}[ht]
% \centering
% \caption{The performance changes wrt. K shots on CONLL2003}
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|cccc}
% \toprule

% \multirow{2}{*}{Method} &
% \multicolumn{4}{c}{Shots (4 Slot Types)}\\

% \cline{2-5}
%  & 
% 5  & 10 & 20 & 100\\
% \midrule
% \midrule
% BERT (base) & 63.87 & 68.70.71/71.59 & 73.57 &84.36\\
% BERT(Full) & 92.40  & 92.40 & 92.40 & 92.40\\
% \midrule
% CVT & 51.15 &54.03 /54.58 &66.11&81.99\\
% SeqVAT & 58.02 & 68.59/69.14/66.37&74.15&82.20\\
% Mean Teacher &59.04 & 68.67 /68.68  &72.62&84.17\\
% VAT & 57.03 & 65.89/64.17&72.69&84.43\\
% Classic ST & 64.04 & 69.78/72.21 &74.65&84.93 \\
% BOND &62.52  & 67.79/71.32 &74.19&83.87\\
% \midrule
% MetaST &71.49&75.48/77.11/75.62 & 78.54 & 85.77 \\

% \bottomrule
% \end{tabular}
% }

% \end{table}


\begin{table}[ht]
\centering
\caption{Wikiann Dataset (English).} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (3 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 37.01 & 45.61 & 54.53 & 67.87\\
BERT(Full) & 84.04   & 84.04  & 84.04 & 84.04 \\
\midrule
CVT &16.05 & 27.89/29.75 & 46.42&66.36\\
SeqVAT & 21.11 & 35.16&42.26&62.37\\
Mean Teacher & 30.92 & 41.43 & 50.61 & 67.16\\
VAT & 24.72 & 38.81 & 50.15 & 66.31\\
Classic ST & 32.72 & 46.15 & 54.41 & 68.64\\
BOND & 34.22 & 48.73 & 52.45 & 68.89 \\
\midrule
MetaST &55.04& 57.01/52.18/59.31 & 60.38 & 73.20\\

\bottomrule
\end{tabular}
}

\end{table}




\begin{table}[ht]
\centering
\caption{Multilingual CONLL2003 Dataset.} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (4 Slot Types)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 0.6480 & 0.7077/72.33 & 0.7389 & 0.8061 \\
BERT(Full) & 0.8767 & 0.8767& 0.8767 & 0.8767 \\
\midrule

Mean Teacher & 0.6455 &0.6834&0.7387&0.7921\\
VAT &0.6497 & 0.6763 & 0.7426 & 0.8070  \\
Classic ST &0.6795 &  0.7269&0.7379&0.8182\\
BOND & 0.6942 & 0.7279 & 0.7602 & 0.8062  \\
\midrule
MetaST &0.7334 &  76.65 & 77.01 & 82.11\\

\bottomrule
\end{tabular}
}

\end{table}

\begin{table}[ht]
\centering
\caption{Multilingual Wikiann Dataset.} 
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Method} &
\multicolumn{4}{c}{Shots (3 Slot Types $\times$ 41 languages)}\\

\cline{2-5}
 & 
5  & 10 & 20 & 100\\
\midrule
\midrule
BERT (base) & 0.7768 & 0.7967/77.02/77.35 & 0.8233 & 0.8570 \\
BERT(Full) &  0.8717 &  0.8717 &  0.8717 & 0.8717 \\
\midrule

Mean Teacher & 0.7709 & 0.8023 & 0.8219 & 0.8534\\
VAT & 0.7471 & 0.7882 & 0.8260 & 0.8582\\
Classic ST & 0.7673  & 0.8024 & 0.8239 & 0.8608\\
BOND & 0.7881 & 0.7957 & 0.8219&0.8614 \\
\midrule
MetaST &79.10& 81.47/81.75/81.11 & 83.14 & 85.57\\

\bottomrule
\end{tabular}
}

\end{table}




